LightPainter: Interactive Portrait Relighting with Freehand Scribble

Recent portrait relighting methods have achieved realistic results of portrait lighting effects given a desired lighting representation such as an environment map. However, these methods are not intuitive for user interaction and lack precise lighting control. We introduce LightPainter, a scribble-based relighting system that allows users to interactively manipulate portrait lighting effect with ease. This is achieved by two conditional neural networks, a delighting module that recovers geometry and albedo optionally conditioned on skin tone, and a scribble-based module for relighting. To train the relighting module, we propose a novel scribble simulation procedure to mimic real user scribbles, which allows our pipeline to be trained without any human annotations. We demonstrate high-quality and flexible portrait lighting editing capability with both quantitative and qualitative experiments. User study comparisons with commercial lighting editing tools also demonstrate consistent user preference for our method.

==> tables/ab_two_step.tex <==

\begin{table}[t]
       
        \small
        %\scriptsize
        \centering
        \caption{Ablation study on two-step relighting scheme}
         \vspace{-3mm}
        \tabcolsep=0.1cm
        \resizebox{\columnwidth}{!}{
                %\hspace{-0.5cm}
                \begin{tabular}{l|cc|c|cc}
                        \hline
                        Methods       & LPIPS$\downarrow$   &NIQE$\downarrow$    & Deg.$\uparrow$   & PSNR$\uparrow$  & SSIM$\uparrow$  \\ \hline
                        One-Step          &0.1423 &7.691 &0.8874 &23.88 &0.5278 \\ 
                        
                        \textbf{Two-Step (ours)} & \textbf{0.0848}  & \textbf{7.012}& \textbf{0.9310}&\textbf{28.48}  &\textbf{0.8899} \\ \hline
                        
        \end{tabular}}\label{tab:ab-step}
        \vspace{-4mm}
\end{table}


